Anomalously large relaxation times in dissipative lattice models beyond the non-Hermitian skin effect

We show for generic quantum non-Hermitian tight-binding models that relaxation timescales of local observables are not controlled by the localization length $\xi_{\rm loc}$ associated with the non-Hermitian skin effect, contrary to popular belief. Instead, interference between eigenvectors effectively makes the extreme localization of modes largely irrelevant to relaxation; this is ultimately a consequence of causality and locality. Focusing on the paradigmatic Hatano-Nelson model, we demonstrate that there exists instead a much larger length scale $\xi_{\rm prop}$ which controls the rate of decay towards the steady state. Further, varying $\xi_{\rm prop}$ can lead to anomalously large relaxation times that scale with system size, or to the expected behavior where the dissipative gap correctly predicts the rate of decay. Our work highlights an important aspect of the non-Hermitian skin effect: the exceptional sensitivity to boundary conditions here necessarily takes a finite amount of time to manifest itself.

==> main_text_only.tex <==
\begin{abstract}
We show for generic quantum non-Hermitian tight-binding models that relaxation timescales of local observables are not controlled by the localization length $\xi_{\rm loc}$ associated with the non-Hermitian skin effect, contrary to popular belief. Instead, interference between eigenvectors effectively makes the extreme localization of modes largely irrelevant to relaxation; this is ultimately a consequence of causality and locality. Focusing on the paradigmatic Hatano-Nelson model, we demonstrate that there exists instead a much larger length scale $\xi_{\rm prop}$ which controls the rate of decay towards the steady state. Further, varying $\xi_{\rm prop}$ can lead to anomalously large relaxation times that scale with system size, or to the expected behavior where the dissipative gap correctly predicts the rate of decay. Our work highlights an important aspect of the non-Hermitian skin effect: the exceptional sensitivity to boundary conditions here necessarily takes a finite amount of time to manifest itself.   
\end{abstract}

\maketitle
\emph{Introduction -- } The exotic effects of non-Hermiticity in classical and quantum systems alike has generated widespread interest in recent years \cite{Okuma_2022_NH_review, Ashida_2020_NH_review, Bergholtz_2021_RMP_NH_review}. One such unusual phenomenon is the existence of anomalously long relaxation times: generic local observables reach their steady-state value much more slowly than the characteristic decay rates, the smallest of which is known as the dissipative gap, would suggest \cite{wolf_math_phys_paper, Song_2019_PRL_chiral_damping}. This behavior has been observed in a wide range of  models such as random quantum circuits \cite{Bensa_PRX_2021_randcircs, Znidaric_2022_arxiv_randcirc_NHSE, Bensa_PRR_2022_two_step_phantom, Claeys_2022_randcirc} and non-Hermitian tight-binding models \cite{Haga_PRL_2021_LSE, Mori_PRL_2020_LSE, Yang_2022_PRR}. The latter %, wherein particle propagation on a lattice is dictated by a non-Hermitian Hamiltonian, 
also exhibits counter-intuitive behavior known as the non-Hermitian skin effect (NHSE) \cite{NHSE_ref_1, NHSE_ref_2, NHSE_ref_3, Kunst_2018_PRL_biorth_correspondence}, which occurs when the Hamiltonian under open boundary conditions has a macroscopic number of localized edge modes and a drastically different spectrum than its periodic boundary condition counterpart. The NHSE has been probed in experiments \cite{Coulais2019, liang2022_nhexpt, wang2022_nhexpt}. 

Recent work has suggested that these two counterintuitive effects are in fact intimately related. By interpreting a Lindblad superoperator as a non-Hermitian Hamiltonian, Ref.~\cite{Haga_PRL_2021_LSE} argues that exponentially-large-in-system-size expansion coefficients due the NHSE leads to a unexpectedly-large relaxation time 
\begin{align}\label{eq:naive_relaxation_intro}
\tau_{\rm EVec}
% {\overset{\text{EVec pred.
% }}{\sim}}
{\sim}
 \frac{L}{\xi_{\rm loc} \Delta},
\end{align}
where $\tau$ is a reasonably-defined relaxation timescale for a local observable, $L$ is the size of the system, $\Delta$ is the dissipative gap \cite{Minganti2018_PRA_Liouvillian_diss_gap}, and $\xi_{\rm loc}$ is the localization length of the corresponding least-damped Liouvillian eigenmode. Since the argument leading to Eq.~(\ref{eq:naive_relaxation_intro}) is based solely on the localized Lindblad eigenvectors, we refer to it as the eigenvector (EVec) prediction. A similar argument was put forth in Refs.~\cite{Mori_PRL_2020_LSE, Mori_PRR_2021_MB_explosion}. 

\indent In this Letter, we argue that this analysis is not valid for generic 1D non-Hermitian tight-binding models;
not only is the relaxation time insensitive to $\xi_{\rm loc}$, but $\tau \Delta$ need not even scale with $L$. The mechanism leading to the breakdown of Eq.~(\ref{eq:naive_relaxation_intro}) is simple but ubiquitous in tight-binding models exhibiting the NHSE: the dynamics of local observables involve a large number of eigenvectors, and interference between these modes can effectively make their exponentially-localized nature largely irrelevant. This conclusion, unlike the prediction of Eq.~(\ref{eq:naive_relaxation_intro}), cannot be reached by considering the eigenvectors or eigenvalues separately. Rather, the combination of both is essential to understand the physics at play, as is done naturally when one considers the system's Green's functions.  While we focus on a few well-studied models (the quantum realization of the Hatano-Nelson model \cite{OG_QHN_1, OG_QHN_2} and two additional models in \cite{SM}) for concreteness, we argue that this cancellation is generic and must occur due to locality and causality. 
Note that one can also study anomalous relaxation in non-Hermitian models using pseudo-spectra methods \cite{Flynn_2021_majorana_bosons, Okuma_Sato_PRB_2020_pseudospectra, Znidaric_2022_arxiv_randcirc_NHSE}; however, these do not generally allow one to make precise statements, nor do they provide the intuition we present here.

\begin{figure*}[htpb]
    \centering
    \includegraphics[width=\linewidth]{fig_1_main_text_v4.png}
    \caption{(a) Schematic of the quantum Hatano-Nelson (QHN) model realized using engineered dissipation with hopping amplitudes $w\pm \kappa$, local pumping $\Gamma$ and local loss $\lambda+\kappa$. 
    (b) Normalized relaxation time $\tau_{L, {\rm b}} \Delta_{\rm b}$ (c.f.~Eq.~(\ref{eq:boson_scaling})) for bosons, for various $\Gamma$  in the highly non-reciprocal limit $w = 1, \kappa = 0.999$ leading to a fixed localization length $\xi_{\rm loc} = 0.26 $. The EVec prediction $\tau_{\rm b}\Delta_{\rm b} \sim L/\xi_{\rm loc}$ gets the linear in $L$ scaling correct but dramatically overestimates the prefactor.
    (c) Same as (b) but for fermions. Here, the linear-in-$L$ scaling of the EVec prediction is qualitatively wrong, with $\tau_{L, {\rm b}} \Delta_{\rm b}$ saturating with $L$.  
    As discussed in the main text, these strong deviations from the EVec prediction arise from an interference effect. 
    (d) $\tau_{L,{\rm f/b}}\Delta_{\rm f/b}$  as a function of local loss for $w = 1$, $\kappa = 0.999$, $\Gamma = 0.05$. Changing $\lambda$ does not change $\xi_{\rm loc}$ (the NHSE is unaffected), but strongly modifies 
    $\tau_{L,{\rm f/b}}$; this again strongly disagrees with the EVec prediction.  For large $\lambda$, we recover the behaviour of a reciprocal chain with the dissipative gap correctly predicting the relaxation time.
    } 
    \label{fig:perf_nr_plots}
\end{figure*}

\bigskip

\emph{Quantum Hatano-Nelson model -- } The Hatano-Nelson model is a paradigmatic model exhibiting the NHSE. It can be realized in an unconditional, fully quantum setting using engineered dissipation  \cite{Metelmann_2015_PRX_nr_reseng}. The most natural realization is through the use of nearest-neighbour correlated loss \cite{AM_QHN_paper, liang2022_nhexpt}. The equation of motion for the density matrix using this setup reads (setting $\hbar = 1$)
\begin{align}\nonumber
     \partial_t \hrho
    & =
    -i\frac{w}{2}
    \sum_{j=1}^{L}
    [
    \hc_{j+1}^\dagger \hc_j + \text{h.c.}, \hrho
    ]
    +\kappa
    \sum_{j=1}^{L-1} 
    \mathcal{D}[\hc_j-i\hc_{j+1}]\hrho
    \notag \\ \label{eq:L_HN}
    &\qquad  
%    \kappa \left( \mathcal{D}[\hc_1] + \mathcal{D}[\hc_L] \right) \hrho + 
    + 2   \sum_{j=1}^L \lambda_j \mathcal{D}[\hc_j]\hrho 
    +
    2\Gamma \sum_{j=1}^L\mathcal{D}[\hc_j^\dagger]\hrho
        \equiv
    \mathcal{L} \hrho,
\end{align}
where we consider an $L$-site lattice, open boundary conditions, 
and
$\lambda_j = \lambda + \kappa \left( \delta_{j,1} + \delta_{j,L} \right)$
\footnote{Note that the extra loss $\kappa$ maintains translational invariance on the chain: the local loss on each site is now exactly $\kappa + \lambda$.}.
Here $w$ is the coherent hopping strength, $\mathcal{D}[\hat{X}]\hrho \equiv \hat{X}\hrho \hat{X}^\dagger - \{\hat{X}^\dagger \hat{X}, \hrho\}/2$ is the usual dissipator, $\mathcal{L}$ is the Liouvillian superoperator, and $\hc_j$ are fermionic or bosonic annihilation operators for site $j$; we analyze both cases simultaneously. The degree of non-reciprocity can be tuned by varying the correlated loss $\kappa$. This becomes explicit in the equations of motion for the covariance matrix:
\begin{equation}\label{eqn:EOM}
\begin{aligned}
    &i \partial_t \langle \hat{c}_n^{\dag} \hat{c}_m \rangle 
    = 
    \\  
    & \sum_{j=1}^L
    \left( 
    (\mathbb{H}_{\rm HN} )_{mj} \langle \hat{c}_n^{\dag} \hat{c}_j \rangle 
    - 
    ( \mathbb{H}_{\rm HN}^{\dag} )_{jn} \langle \hat{c}_j^{\dag} \hat{c}_m \rangle  
    \right) 
    + 
    i 2\Gamma \delta_{nm}
    ,
\end{aligned}
\end{equation}
with $\mathbb{H}_{\rm HN}$ is the first-quantized Hatano-Nelson Hamiltonian
\begin{equation}
\begin{aligned}\label{eq:HN_Matrix}
\mathbb{H}_{\rm HN} \equiv 
&\sum_{j=1}^{L-1}
\left( 
\frac{w + \kappa}{2} | j + 1 \rangle \langle j |  
+  \frac{w - \kappa}{2} | j \rangle \langle j + 1 | 
\right) 
\\&-  i ( \kappa + \lambda \pm  \Gamma ) \sum_{j=1}^L|j\rangle \langle j|.
\end{aligned}
\end{equation}
Throughout, we will use the upper and lower sign $\pm$ for fermions and bosons respectively in addition to fixing $w \geq 0$ and $w> \kappa$, ensuring that the left-to-right hopping amplitude is stronger than right-to-left hopping. Note that the local loss proportional to $\kappa$ cannot be avoided if we want non-reciprocity. Without it, we could violate Pauli exclusion or the Heisenberg uncertainty principle \cite{Clerk_2010_RMP_noise_review}. The extra local loss $\lambda$ thus allows us to vary the degree of non-reciprocity without changing the total local loss. Incoherent pumping $\Gamma$ ensures the existence of a steady state with a finite density of particles with a non-trivial spatial profile \cite{AM_QHN_paper}. Finally, note that $\mathbb{H}_{\rm HN}$ is distinct from the no-jump Hamiltonian \cite{gardiner_zoller_2010}.

In what follows, we will be interested in the relaxation time of local observables. Given that the non-reciprocal hopping in Eq.~(\ref{eq:HN_Matrix}) favors rightward propagation and we wish to consider the effects of system size on relaxation dynamics, it is  natural to consider the occupation of the rightmost site $\langle \hat{n}_L(t) \rangle$. We define the normalized non-equilibrium population $\delta n_L(t) = \left| \langle \hat{n}_L(t) \rangle - \langle \hat{n}_L(\infty) \rangle \right|  / \langle \hat{n}_L(\infty) \rangle$ and for concreteness assume that the chain starts in vacuum: $\delta n_L(0) = 1$. To define a local relaxation time $\tau_L$, we fix a relaxation threshold $e^{-1}$, and say that site $L$ has relaxed at time $\tau_L$ when $\delta n_L(\tau_L) = e^{-1}$. The essential physics we discuss is not specific to the local observable of interest, initial state or choice of reasonable relaxation threshold. See \cite{SM} for a discussion of other initial conditions, and the full time-dependent decay curve.  

\bigskip

\emph{Exponentially large coefficients -- } To solve Eq.~(\ref{eqn:EOM}) and extract $\tau_L$, we first diagonalize $\mathbb{H}_{\rm HN}$. The eigenvalues $E_{\alpha}$ and biorthonormal left and right eigenvectors $\langle \psi^l(\alpha) | \psi^r(\beta) \rangle = \delta_{\alpha \beta}$ of the Hatano-Nelson model are well known \cite{OG_QHN_1, OG_QHN_2}. We have $E_\alpha = J \cos k_\alpha-i(\kappa + \lambda \pm \Gamma)$ and 
\begin{align}\label{eq:Eigenvectors}
    \langle j|\psi^{r(l)}(\alpha) \rangle\equiv
    \psi_j^{r(l)} (\alpha) = 
    \sqrt{\frac{2}{L+1}}
    e^{(-) j/\xi_{\rm loc}} \sin k_\alpha j
\end{align}
% \AC{A bit confusing as $\pm$ used already for fermions versus bosons....}
with
\begin{align}\label{eq:J_xi_def}
    J \equiv \sqrt{(w+\kappa)(w-\kappa)}
    ,
    \: 
    e^{1/\xi_{\rm loc}}
    \equiv
    \sqrt{\frac{w+\kappa}{w-\kappa}}.
\end{align}
Here, $k_\alpha = \alpha\pi/(L+1), \alpha = 1, \dots, L$ is a quantized standing-wave momentum. The parameter $J$ should be thought of as a renormalized hopping amplitude, whereas $\xi_{\rm loc}$ is not only the localization length of the eigenvectors but serves as a measure of non-reciprocity. We stress that fermions and bosons have the same eigenvectors, and the only difference between the two is the uniform decay rate $\Delta_{\rm f/b} \equiv - {\rm Im} E_{\alpha} = \kappa + \lambda \pm \Gamma$. Having diagonalized $\mathbb{H}_{\rm HN}$, we can use third quantization to also diagonalize the full Liouvillian \cite{Prosen_3Q, Prosen_2010, AM_2022_unpublished}, analogous to how one diagonalizes a second-quantized quadratic Hamiltonian from its single-particle data. The eigenvalues of $\mathcal{L}$ are fully determined by $E_{\alpha}$ and its eigenmodes are simply related to the left and right eigenvectors of $\mathbb{H}_{\rm HN}$ and the steady-state correlation matrix $(\mathbb{S})_{nm} \equiv \langle \hc^\dagger_n \hc_m \rangle_{\rm ss}$.

We can now use the spectral decomposition of $\mathbb{H}_{\rm HN}$ to formally express $\langle \hat{n}_m(t) \rangle$ as a sum over eigenvectors 
\begin{equation}\label{eqn:formal_soln}
\begin{aligned}
    &\langle \hat{n}_m(t) \rangle 
    =
    2 \Gamma  \sum_{j=1}^m \int_{0}^{t} dt' 
    \left|
    \langle m | e^{-i \mathbb{H}_{\rm HN}(t-t')} |j \rangle
    \right|^2
    \\
    = 
    &2 \Gamma  
    \sum_{j=1}^m
    \int_0^t
    dt'
    \left|
    \sum_{\alpha}
    \psi^r_m(\alpha) (\psi^l_j(\alpha))^* e^{-i E_\alpha (t-t')}
    \right|^2.
    \\
    &
\end{aligned}
\end{equation}
 Eq.~(\ref{eqn:formal_soln}) provides a simple physical picture of the dynamics. At some time $ t' \leq t$, a pump bath attached to site $j$ injects a particle, which then propagates to a site $m$ in a time $t-t'$ contributing $P(m, j; t-t') \equiv |\langle m | e^{-i \mathbb{H}_{\rm HN}(t-t')} |j \rangle|^2 $ to the density at that site. With each bath adding particles at a rate $2\Gamma$, and considering we started in vacuum at time $t = 0$, summing over all sites $j$ and integrating over all intermediate times $t'$ gives the total particle number on site $m$. Henceforth we will focus mainly on the rightmost site $m = L$.
% \AC{Should we write Eq. 7 for a general site m?  This matches the text better.}

With the propagator $\langle L | e^{-i \mathbb{H}_{\rm HN} t} | j \rangle$ written in its spectral representation, from Eq.~(\ref{eq:Eigenvectors}) it seems apparent that for strong non-reciprocity $\kappa \to w$, $\xi_{\rm loc} \ll 1$, only particles injected on the first site $j= 1$ which propagate to site $L$ matter, since in this limit the $e^{2(L-1)/\xi_{\rm loc}}$ factor in this term (coming from the exponential localization of the right eigenvectors) will dominate over all others.  To estimate $\tau_L$, one might then argue that we must compare this large term with $e^{- \Delta_{\rm f/b} t}$, the temporal decay stemming from the imaginary part of the mode energies.   $\tau_L$ is then roughly the time it takes for the temporal decay factor to cancel the exponentially-large expansion coefficient. We would thus approximately have
\begin{align}\label{eqn:naive_relaxation}
\tau_{L, \rm f/b}
\stackrel{?}{\sim}
 \frac{L}{\xi_{\rm loc} \Delta_{\rm f/b}}.
\end{align}
This is essentially the argument put forward in Refs.~\cite{Haga_PRL_2021_LSE, Mori_PRL_2020_LSE}. We show this explicit connection in \cite{SM} by demonstrating that the exponentially-large terms in Eq.~(\ref{eqn:formal_soln}) are related to expansion coefficients in the basis of Liouvillian eigenmodes. 

In Fig.~\ref{fig:perf_nr_plots}(b) and (c) we plot $\tau_L$ in the large non-reciprocal limit $\kappa = 0.999 w$ giving $\xi_{\rm loc} = 0.26$ and, for $L = 100$, an expansion coefficient of $e^{2(L-1)/\xi_{\rm loc}} \sim 10^{330}$ \footnote{One might argue that a localization length $\xi_{\rm loc}$ much smaller than the lattice constant cannot reasonably be considered a physical quantity. In \cite{SM}, we show that Eq.~(\ref{eqn:naive_relaxation}) is wrong even for $\xi_{\rm loc} \sim O(1)$.}. Clearly the EVec prediction Eq.~(\ref{eqn:naive_relaxation}) is not even qualitatively correct. Not only is the relaxation time sensitive to the small incoherent pumping $\Gamma$, but for fermions $\tau_L$ saturates for large enough system sizes, and we do not recover the predicted linear-in-$L$ scaling. While appealing, the argument leading to Eq.~(\ref{eqn:naive_relaxation}) is clearly misleading; we diagnose and correct the crucial error in what follows.

\bigskip

\emph{Interference between eigenmodes -- } The failure of Eq.~(\ref{eqn:naive_relaxation}) makes it evident that we cannot simply estimate the magnitude of the propagator using the localization properties of the eigenvectors. To understand why, first note that Eq.~(\ref{eq:Eigenvectors}) implies $ \langle m | e^{-i \mathbb{H}_{\rm HN} t} |j \rangle = e^{(m-j)/\xi_{\rm loc}- \Delta_{\rm f/b} t} \langle m | e^{-i \mathbb{H}_{J} t} |  j \rangle$ where $\mathbb{H}_{J}$ is a \textit{reciprocal} nearest-neighbour tight-binding Hamiltonian with hopping amplitude $J$ under open boundary conditions. Focusing on the impact of this  previously-ignored second factor, we now work in the strongly non-reciprocal limit $\kappa \rightarrow w$ and set $\lambda = 0$, just as in Fig.~(\ref{fig:perf_nr_plots}) . In this limit, leftwards propagation is strongly suppressed. A particle which hits the right-most edge of the chain essentially cannot be reflected back and affect any other site; the boundary becomes irrelevant. Estimating the propagator by its fully translationally-invariant counterpart gives
\begin{align}\label{eq:Approx_P}
&P(L, j; t)
\approx
e^{2(L-j)/\xi_{\rm loc}-2 \Delta_{\rm f/b} t}
\left|
\int_{-\pi}^{\pi}
\frac{d k}{2\pi}
e^{i k(L-j)}
e^{-i J \cos k t}
\right|^2
\end{align}
and we show in \cite{SM} that this is in fact an excellent approximation in the regime of interest. 

Using Eq.~(\ref{eq:J_xi_def}) we deduce that although the first factor of Eq.~(\ref{eq:Approx_P}) is enormous for $j \ll L$ and strong reciprocity (i.e.~$\xi_{\rm loc} \ll 1$), the second factor in this limit can be very small,  as $J \to 0$. In fact, expanding to lowest order in $J$ and expressing all quantities in terms of $w$ and $\kappa$:
\begin{align}\nonumber
P(L,j;t)
&\approx 
\left(
J
e^{1/\xi_{\rm loc}}
\right)^{2(L-j)}
\frac{
e^{-2\Delta_{\rm f/b}t}
t^{2(L-j)}
}
{
4^{L-j}([L-j]!)^2
}
\\ \label{eq:Approx_P_Simplified}
&
=
\left(
w+\kappa
\right)^{2(L-j)}
\frac{
e^{-2\Delta_{\rm f/b}t}
t^{2(L-j)}
}
{
4^{L-j}([L-j]!)^2.
}
\end{align}
We see explicitly that the exponentially-large contribution from $\xi_{\rm loc}$ has been offset by the small renormalized hopping amplitude. 

The above dramatic cancellation is due to the interference between the eigenvectors of the Hatano-Nelson model, as in Eq.~(\ref{eq:Approx_P_Simplified}) we have summed over all $\alpha$ in the spectral decomposition of the propagator $\langle L|e^{-i \mathbb{H}_{\rm HN}t}|j\rangle = \sum_{\alpha} \psi^r_L(\alpha) (\psi^l_j(\alpha))^* e^{-i E_\alpha t}$. Indeed, before Eq.~(\ref{eqn:naive_relaxation}) we incorrectly estimated the magnitude of $P(L,j;t)$ because we focused on a {\it single} eigenvector.  This incorrectly neglects the fact 
that for $J \to 0$, we have many modes with closely spaced eigenvalues $E_{\alpha}$, and the possibility of destructive interference when we sum their contributions.  While this explanation might seem mechanistic, it has a more general physical underpinning.  
This cancellation had to occur to enforce locality: a particle injected at $j \ll L$ cannot instantaneously propagate to $L$ with an exponentially-large amplitude, and hence cannot instantaneously know about the exponential modification of wavefunctions associated with the boundary condition.  We expand on this point in the next section, arguing that this reasoning also holds for intermediate times and is not limited to the Hatano-Nelson model. 

Despite demonstrating that the localization length plays no role in determining the relaxation time, it still does not explain why $\tau_L$ displays qualitatively different behavior for fermions and bosons nor why it is sensitive to the small incoherent pumping rate $\Gamma$. To uncover the origin of this effect, for simplicity consider the perfectly non-reciprocal case $\kappa = w$ where the dissipative gap takes the form $\Delta_{\rm f/b} = w \pm \Gamma$ and Eq.~(\ref{eq:Approx_P_Simplified}) is exact \footnote{Although this corresponds to an exceptional point pf $\mathbb{H}_{\rm HN}$, this structure is irrelevant here since the propagator $e^{-i \mathbb{H}_{\rm HN} t}$ is a smooth function of $\mathbb{H}_{\rm HN}$ and its parameters. Our conclusion holds for strong but not perfect non-reciprocity, just as in Fig.~(\ref{fig:perf_nr_plots})}. Fixing the distance $L-j$, a simple calculation reveals that $P(L,j;t)$ is a sharply-peaked function in the time domain, being maximal at
\begin{align}\label{eq:crit_t}
    t^{\max}_{L-j}
    \equiv
    \frac{L-j}
    {w\pm \Gamma} = \frac{L-j}
    {\Delta_{\rm f/b}}.
\end{align}
As shown in \cite{SM}, qualitatively it is correct to neglect the temporal integral in Eq.~(\ref{eqn:formal_soln}) and think about a particle injected at site $j$ as arriving at site $L$ at time $t^{\rm max}_{L-j}$ and contributing $P(L, j; t^{\rm max}_{L-j})$ to $\langle \hat{n}_L(t) \rangle$. 
We can interpret $t_{L-j}^{\rm max}$ as the effective time it takes for a particle to propagate a distance $L-j$. 


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig_2_main_text_v5.pdf}
    \caption{Schematic representation of particle propagation in the lattice. 
    (a) Fermions injected into the chain are de-amplified as they propagate to the right. Consequently, the primary contributions to the final site $L$ come from a small range of nearby sites within a distance $\xi^{\rm{f}}_{\rm prop}$ of the end of the chain. 
    (b) Bosons injected into the chain are amplified as they propagate to the right.
    Consequently, the primary contributions to the final site $L$ come from a small range of sites within a distance $\xi^{\rm{b}}_{\rm prop}$ of the start of the chain. 
    These processes set the decay time $\tau_{L}$; see Eqs.~(\ref{eq:fermion_scaling})-(\ref{eq:boson_scaling}) and accompanying discussion. } 
    \label{fig:prop_schematic}
\end{figure}

Surprisingly, depending on the type of particle, the amplitude $P(L,j;t) = |\langle L | e^{-i\mathbb{H}_{\rm eff} t}|j \rangle|^2$ evaluated at its peak has a strikingly different spatial behavior
\begin{align}\label{eq:P_max}
    P(L,j; t^{\max}_{L-j})
    \propto
    \left(
    \frac{w}{w\pm \Gamma}
    \right)^{2(L-j)}
    \equiv
    e^{\mp(L-j)/\xi_{\rm prop}^{\rm f/b}}
    .
\end{align}
As a function of distance $L-j$, we thus have exponential \textit{growth} (amplification) for bosons, whereas for fermions we have the opposite: exponential \textit{decay} (attenuation). The length scale controlling this behavior is not $\xi_{\rm loc}$ but rather $(\xi_{\rm prop}^{\rm f/b})^{-1} = \mp 2\ln(w/(w\pm \Gamma)) >0$. For fermions, this attenuation means that only particles injected within a length $\xi_{\rm prop}^{\rm f}$ of the left site $L$ can reach it; adding additional sites on the leftmost side of the chain effectively does not change $\langle \hat{n}_L \rangle_{\rm ss}$. Using Eq.~(\ref{eq:crit_t}), we must then only wait a time 
\begin{align}\label{eq:fermion_scaling}
    \tau_{L, \rm f}
    \sim
   t^{\max}_{\xi_{\rm prop}^{\rm f}}
    \approx
    \frac{\xi_{\rm prop}^{\rm f}}{\Delta_{\rm f}}
\end{align}
before all particles in the steady state are accounted for, explaining the saturation we see in Fig.~(\ref{fig:perf_nr_plots}c). For bosons however the amplification physics implies that, for large $L$, particles on the first site contribute the \textit{most} to the occupation on the last site. Consequently, we must wait for a particle injected on the first site to propagate the length of the chain leading to 
\begin{align}\label{eq:boson_scaling}
    \tau_{L, \rm b}
    \sim
    t^{\max}_{L-1}
    \approx
    \frac{L}{\Delta_{\rm b}}.
\end{align}
This analysis is corroborated by Fig.~(\ref{fig:perf_nr_plots}b) of the main text, and Fig.~(\ref{fig:fermion_sat_fit}) in \cite{SM}. This is another main result of this work: amplifying and decaying dynamics have markedly different relaxation behavior. The intuitive picture of propagation for both types of particles are schematically depicted in Fig.~(\ref{fig:prop_schematic}).

\emph{Generic tight-binding Hamiltonians -- } 
It is natural to ask whether the relaxation behaviour of the quantum Hatano-Nelson model is generic. Suppose now that we have realized a short-ranged non-Hermitian tight-binding Hamiltonian $\mathbb{H}_{\rm eff}$ exhibiting the NHSE using engineered Markovian dissipation, in the sense that the dynamics of the covariance matrix obey Eq.~(\ref{eqn:EOM}), perhaps with a different inhomogeneous term. Under open boundary conditions, the eigenvectors and eigenvalues of $\mathbb{H}_{\rm eff}$ are $\psi^{r(l)}_{\boldsymbol{m} \boldsymbol{\sigma}}(\alpha) \sim e^{(-) \boldsymbol{m}/\xi_{\alpha}}$ and $E_{\alpha}$ respectively, where $\boldsymbol{m}$ denotes a site of an arbitrary-dimensional lattice, $\boldsymbol{\sigma}$ indexes all other degrees of freedom and $\xi_{\alpha}$ is the localization length of mode $\alpha$. The propagator in the position basis $\langle \boldsymbol{m} \boldsymbol{\sigma}|
e^{-i \mathbb{H}_{\rm eff} t} 
| \boldsymbol{j} \boldsymbol{\sigma'} \rangle 
= 
\sum_{\alpha} 
\psi^{r}_{\boldsymbol{m} \boldsymbol{\sigma}}(\alpha)
(\psi^{l}_{\boldsymbol{j} \boldsymbol{\sigma'}}(\alpha))^*
e^{- iE_{\alpha} t}
$
can be used to determine any local observable, just as in Eq.~(\ref{eqn:formal_soln}). How can we generically conclude that the eigenvectors will interfere and render the relation dynamics largely insensitive to $\xi_{\alpha}$? 

Ultimately, the answer is locality and causality. For a sufficiently local Hamiltonian particles have a finite propagation speed i.e.~a Lieb-Robinson velocity \cite{Lieb_1972_LR_bound}. For sites $\boldsymbol{m}, \boldsymbol{j}$ well within the bulk, there is thus a timescale over which the presence or absence of the boundaries is essentially irrelevant. In this regime we can thus approximate the Green's functions of the OBC system by its infinite-sized counterpart using plane-waves, just as we did in Eq.~(\ref{eq:Approx_P}). Any important length scale can thus be deduced from the spectrum and eigenvectors of the periodic-boundary-condition chain. This is the case for the model presented above: $\xi_{\rm loc}$ drops out of the expression of the Green's function for an infinite chain, whose relevant length scale is instead $\xi_{\rm prop}^{\rm f/b}$.

The spectral decomposition however is of course exact for all times; the eigenvectors and eigenvalues are after all effectively infinitely-temporally resolved objects.  The only way to obtain recover both locality and a macroscopic number of spatially-localized edge modes is a large cancellation between eigenvectors at intermediate times. In a sense, although the NHSE drastically changes the spectrum and eigenvectors of $\mathbb{H}_{\rm eff}$, they must change together in just the right way to render the local propagation physics effectively the same. The exponential sensitivity to boundary conditions is thus not an instantaneous effect.

\bigskip

\emph{Conclusion -- } We have demonstrated that while non-Hermitian models exhibiting the NHSE can exhibit anomalous relaxation times, this is not in general simply determined by the localization length of eigenvectors.  This can be understood as resulting from an interference effect, and more generally on considerations involving locality and causality (which limit the sensitivity to changes in boundary conditions).  While our conclusions are based on detailed studies of the quantum Hatano-Nelson model (and two additional setups in \cite{SM}), we believe that they are generic to any local model. Our work also highlights and emphasizes how there is a timescale associated with the presence of boundaries in models exhibiting the NHSE. Future works exploring how the effects of interactions impact this analysis would be extremely interesting, as would attempting to place quantitative bounds on how boundaries affect finite-time dynamics.  

\bigskip

This work was supported by the Air Force Office of Scientific Research MURI program under Grant No. FA9550-19-1-0399, and by the Simons Foundation (Grant No. 669487, A. C.).


